Generating Maximal Configurations and Their Variants Using Code Metrics

Testing configurable systems continues to be challenging and costly. Generation of configurations for testing tends to use either techniques based on semantic sampling (e.g., logical formulas over configuration variables, often called presence conditions) or structural code metrics (e.g., code coverage). In this paper we describe our hybrid approaches that combine these two kinds of techniques to good effect. We present new configuration-generation algorithms that leverage constraint solving (SAT and MaxSAT) and configuration fuzzing, and implement our approach in a configuration-generation framework, CONFIZZ. CONFIZZ both enables the generation of maximal configurations (maximal sets of presence conditions that can be satisfied together) and performs code-metric guided configuration fuzzing. Results from evaluation on BusyBox, a highly configurable benchmark, show that our MaxSAT-based configuration generation achieves better coverage for several code metrics. Results also show that, when high coverage of multiple configurations is needed, CONFIZZ's presence-condition fuzzing outperforms alternatives.

==> additionaldata.tex <==
\begin{comment}
\begin{table*}
\begin{footnotesize}
    \begin{tabular}{c|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r} \toprule
          &  & \multicolumn{7}{c|}{MaxSAT Variants (Scores \& Time)} &  \multicolumn{7}{c|}{Presence Condition Fuzzing (Average Scores \& Time (secs))} \\ \cline{3-16}
         {\bf Comp.} & {\bf \# UPC} & {\bf \#} & {\bf Max} & {\bf Min} & {\bf Med.} & {\bf Mean} & {\bf Std.} & {\bf Time} & {\bf \#} & {\bf Max} & {\bf Min} & {\bf Med.} & {\bf Mean} & {\bf Std.} & {\bf Time}\\ \hline
awk & 65 & 542 & 66 & 1 & 26.0 & 23.90 & 16.77 & & 2272.8 & 55.6 & 0.0 & 18.8 & 23.27 & 16.86 & \\
cmp & 62 & 396 & 74 & 25 & 29.0 & 32.88 & 12.01 & & 2916.6 & 62.6 & 0.0 & 23.0 & 26.44 & 17.21 & \\
diff & 68 & 584 & 73 & 1 & 25.0 & 24.03 & 18.00 & & 2129.0 & 57.0 & 0.0 & 17.6 & 23.19 & 17.59 & \\
ed & 63 & 1183 & 65 & 1 & 25.0 & 23.26 & 8.89 & & 2233.2 & 53.0 & 0.0 & 18.8 & 22.80 & 16.06   \\
patch\_bbox & 65 & 772 & 71 & 2 & 22.0 & 15.78 & 14.98 & & 2042.2 & 58.0 & 0.0 & 17.6 & 23.20 & 17.72 & \\
patch\_toybox & 63 & 1183 & 65 & 1 & 25.0 & 23.26 & 8.89 & & 2169.6 & 56.8 & 0.0 & 18.2 & 23.19   &16.99 & \\
patch & 65 & 772 & 71 & 2 & 22.0 & 15.78 & 14.98 & & 2212.8 & 57.6 & 0.0 & 18.6 & 22.56 & 16.15 & \\
sed & 65 & 1289 & 71 & 1 & 27.0 & 25.31 & 9.45 & & 2273.0 & 56.2 & 0.0 & 19.0 & 23.50 & 16.83 & \\
         \bottomrule
    \end{tabular}
    \end{footnotesize}
    \caption{Comparison of configuration generation approaches for the BusyBox {\em editors} subsystem in terms of the number of generated configurations (\#), maximum, minimum, median, and standard deviation of scores for the LCU metric. UPC denotes the number of unique presence conditions. Fuzzing results are the averages of 5 runs. The fuzzing seed consists of all presence conditions turned off. Number of cycles=3.}
    \label{tab:statcmpeditors}
\end{table*}

\begin{table*}
\begin{footnotesize}
    \begin{tabular}{c|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r} \toprule
          &  & \multicolumn{7}{c|}{MaxSAT Variants (Scores \& Time)} &  \multicolumn{7}{c|}{Presence Condition Fuzzing (Average Scores \& Time (secs))} \\ \cline{3-16}
         {\bf Comp.} & {\bf \# UPC} & {\bf \#} & {\bf Max} & {\bf Min} & {\bf Med.} & {\bf Mean} & {\bf Std.} & {\bf Time} & {\bf \#} & {\bf Max} & {\bf Min} & {\bf Med.} & {\bf Mean} & {\bf Std.} & {\bf Time}\\ \hline
awk & 65 & 542 & 66 & 1 & 26.0 & 23.90 & 16.77 & & 4262.0 & 67.2 & 0.0 & 45.8 & 38.81 & 21.31 & \\
cmp & 62 & 396 & 74 & 25 & 29.0 & 32.88 & 12.01 & & 7178.6 & 71.4 & 0.0 & 43.4 & 40.23 & 19.35  & \\
diff & 68 & 584 & 73 & 1 & 25.0 & 24.03 & 18.00 & & 3976.4 & 71.0 & 0.0 & 48.8 & 40.60 & 22.91 & \\
ed & 63 & 1183 & 65 & 1 & 25.0 & 23.26 & 8.89 & & 4234.4 & 66.8 & 0.0 & 46.0 & 38.64 & 20.84 & \\
patch\_bbox & 65 & 772 & 71 & 2 & 22.0 & 15.78 & 14.98 & & 4465.2 & 70.2 & 0.0 & 46.0 & 39.24 & 21.67 & \\
patch\_toybox & 63 & 1183 & 65 & 1 & 25.0 & 23.26 & 8.89 & & 4153.6 & 65.4 & 0.0 & 45.8 & 38.07 & 20.42 & \\
patch & 65 & 772 & 71 & 2 & 22.0 & 15.78 & 14.98 & & 4126.8 & 70.0 & 0.0 & 47.8 & 40.26 & 22.11 & \\
sed & 65 & 1289 & 71 & 1 & 27.0 & 25.31 & 9.45 & & 4076.6 & 70.6 & 0.0 & 49.0 & 40.52 & 22.73 & \\
         \bottomrule
    \end{tabular}
    \end{footnotesize}
    \caption{Comparison of configuration generation approaches for the BusyBox {\em editors} subsystem in terms of the number of generated configurations (\#), maximum, minimum, median, and standard deviation of scores for the LCU metric. UPC denotes the number of unique presence conditions. Fuzzing results are the averages of 5 runs. The fuzzing seed consists of all presence conditions turned off. Number of cycles=10.}
    \label{tab:statcmpeditors}
\end{table*}

\begin{table*}
\begin{footnotesize}
    \begin{tabular}{c|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r} \toprule
          &  & \multicolumn{7}{c|}{MaxSAT Variants (Scores \& Time)} &  \multicolumn{7}{c|}{Presence Condition Fuzzing (Average Scores \& Time (secs))} \\ \cline{3-16}
         {\bf Comp.} & {\bf \# UPC} & {\bf \#} & {\bf Max} & {\bf Min} & {\bf Med.} & {\bf Mean} & {\bf Std.} & {\bf Time} & {\bf \#} & {\bf Max} & {\bf Min} & {\bf Med.} & {\bf Mean} & {\bf Std.} & {\bf Time}\\ \hline
awk & 65 & 542 & 66 & 1 & 26.0 & 23.90 & 16.77 & & 5737.8 & 67.8 & 0.0 & 54.4 & 45.42 & 21.25 & \\
cmp & 62 & 396 & 74 & 25 & 29.0 & 32.88 & 12.01 & & 8615.6 & 72.0 & 0.0 & 52.4 & 45.86 & 20.35  & \\
diff & 68 & 584 & 73 & 1 & 25.0 & 24.03 & 18.00 & & 5320.6 & 72.0 & 0.0 & 59.2 & 48.12 & 23.31 & \\
ed & 63 & 1183 & 65 & 1 & 25.0 & 23.26 & 8.89 & & 5431.4 & 65.4 & 0.0 & 51.5 & 43.00 & 20.25 & \\
patch\_bbox & 65 & 772 & 71 & 2 & 22.0 & 15.78 & 14.98 & & 5165.4 & 70.4 & 0.0 & 54.4 & 45.60 & 22.12 & \\
patch\_toybox & 63 & 1183 & 65 & 1 & 25.0 & 23.26 & 8.89 & & 5487.2 & 65.4 & 0.0 & 51.6 & 43.02 & 20.15 & \\
patch & 65 & 772 & 71 & 2 & 22.0 & 15.78 & 14.98 & & 6133.6 & 70.2 & 0.0 & 51.8 & 43.93 & 21.55 & \\
sed & 65 & 1289 & 71 & 1 & 27.0 & 25.31 & 9.45 & & 5940.6 & 70.0 & 0.0 & 54.4 & 46.00 & 21.17 & \\
         \bottomrule
    \end{tabular}
    \end{footnotesize}
    \caption{Comparison of configuration generation approaches for the BusyBox {\em editors} subsystem in terms of the number of generated configurations (\#), maximum, minimum, median, and standard deviation of scores for the LCU metric. UPC denotes the number of unique presence conditions. Fuzzing results are the averages of 5 runs. The fuzzing seed consists of all presence conditions turned off. Number of cycles=20.}
    \label{tab:statcmpeditors}
\end{table*}
\end{comment}


==> busyboxFuzzingExperiment.tex <==
%  by Ken

% crashwalk link: https://github.com/bnagy/crashwalk

%   fuzz awk
%  afl-fuzz -i ./input/ -o output/ -- ./busybox awk -f @@  ./a.txt
%  input contains all seeds of awk scripts. They will be changed and replace @@ here. The a.txt is a random txt file.


% fuzz sed
% afl-fuzz -i ./input/ -o output/ -- ./busybox sed -f @@  ./a.txt
%  input contains all seeds of sed scripts. They will be changed and replace @@ here. The a.txt is a random txt file.


% fuzz diff
% afl-fuzz -i ./input/ -o output/ -- ./busybox diff @@  ./a.txt
% the same a.txt file. We also use it as seed in input, to be compared by diff.

% // a.txt
% 1, XXXXXXXX    121   26526   a1213,sadd
% 2, CCCCCCCC    123   951260  2s1#dsad
% 3, DDDDDDDD    423   8512317 212#jon
% 4, ZZZZZZZZ    5245  8654165 323e#plp
% 5, ZZAAAAAA    43213 8546149 213f#asd


We use afl-fuzzing framework to test busybox applet. We select applets that accept file as inputs. For example, awk accept a script as input to process the target text file. We provide the scripts generated from testsuite of busybox as fuzzing inputs.  The variants of scripts that cause crashes detected by fuzzing engine. We tested on three applets, awk, diff and sed. The input of diff command is from a simple crafted file and we use the same file as the input seed to be compared by diff.  The fuzzing of sed command works similarly to awk. The experiment for each afl-fuzzing testcase lasts for 8 hours. Also, we use crashwalk to triage the crashes generated by afl-fuzzing.
 



==> conffuzzing.tex <==



\begin{algorithm}
\begin{algorithmic}[1]
\State {\bf ConfigurationFuzzing}($P$: Presence Conditions, $C$: Cost Function, $SConf$: Seed Configurations, $mode$: \{D, ND, C, IAD, IAND, IAC\}, $N$: Integer, $M$: Num to be filtered)
\State $interMap \gets \lambda v. \{ v' \ | \ p \in P \ \wedge \{v,v'\} \subseteq Vars(p)\}$
\State $PriorityQueue queue \gets \emptyset$
\For{each seed $sc$ in $SConf$}
%   \If{$C=LCU$} \ $score \gets |\{ p \ | \ p \in P \ \wedge \ p \wedge F(sc) \not = false\}|$
%   \Else 
%        \ $score \gets \Sigma_{p \in P, p \wedge F(sc) \not = false, l \in Loc(p)} C(l)$
%   \EndIf
   \State $queue.add(sc, Score(sc,P,C))$
\EndFor     
\State $cycle \gets 1$
\While{$cycle \leq N$ and $queue$ not empty}
   \State $cur \gets queue.removeMax()$
   \If{$mode$ is one of \{D,C,IAD,IAC\}}
      \State Flip each of \{1,2,4\} consecutive bit(s) in $cur$
      \State Add each new (conf,Score(conf,P,C)) to the queue 
   \EndIf
   \If{$mode$ is one of \{ND,C,IAND,IAC\}}
      \State Flip each of \{1,2,4\} random bit(s)  in $cur$
      \State Add each new (conf,Score(conf,P,C)) to the queue 
   \EndIf   
   \If{$mode$ is one of \{IAD,IAC\}}
      \State Flip each $(v_1,v_2)$ s.t. $v_2 \in interMap[v_1]$  in $cur$ 
      \State Add each new (conf,Score(conf,P,C)) to the queue 
   \EndIf  
   \If{$mode$ is one of \{IAND,IAC\}}
      \State Flip each $v_1$ and random $v_2$ s.t. $v_2 \in interMap[v_1]$  in $cur$
      \State Add each new (conf,Score(conf,P,C)) to the queue 
   \EndIf  
\EndWhile
\State {\bf return} Top $M$ confs in queue
\State
\State {\bf Score}($conf$: Configuration, $P$: Presence Conditions, $C$: Cost Function): $\mathcal{N}$
   \If{$C=LCU$} 
     \State {\bf return}  $|\{ p \ | \ p \in P \ \wedge \ p \wedge F(conf) \not = false\}|$
   \Else 
        \State {\bf return} $\Sigma_{p \in P, p \wedge F(conf) \not = false, l \in Loc(p)} C(l)$
   \EndIf
\end{algorithmic}
\caption{Interaction Aware Configuration Fuzzing.}
\label{alg:fuzzing}
\end{algorithm}

\subsection{Configuration Fuzzing}
\label{sec:fuzzing}


The approximate solution to finding the minimum set of configurations given in Section \ref{sec:optimization} is useful but may not scale for large configuration spaces. 
Also, the code metrics may not be sufficient in generating all the configurations that serve the goal of the analysis. 
%Robyn says: add a sentence of explanation, maybe with an example, to motivate the need for configuration fuzzing?
It is then desirable to generate additional configurations starting from a seed set of 
configurations. 
We present a configuration fuzzing that is inspired by the success of 
fuzzing code and tools like AFL \cite{ALF}.
Algorithm \ref{alg:fuzzing} presents our fuzzing approach, which can be 
configured to run in interaction-aware mode (IA) or in interaction-unaware mode. 
Each mode comes with deterministic (IAD and D), nondeterministic (IAND and ND), 
and hybrid (IAC and C) versions.
%Robyn: say "combined" instead of "hybrid" to match C?

One of the inputs to CONFIZZ is the set of presence conditions, $P$, which are 
used to create a configuration interaction map. 
The cost function, $C$, allows us to compute the score for each configuration according 
to the chosen code metric.
If the cost function corresponds to the logical view of code coverage, then 
the score is equal to the number of presence conditions enabled under the given configuration.
Otherwise, the score is equal to the sum of the cost function for each code line that is covered by the enabled presence conditions.

\begin{table}[th!]
    \centering
    \begin{footnotesize}
    \begin{tabular}{l|r|r|r} \toprule
     {\bf Component} & {\bf \# Unique Soft}   & {\bf Covered} & {\bf \# MaxSAT Sol}\\ 
        & {\bf Constraints} &  {\bf Soft Const.} & \\ \hline \hline
         awk   & 69  & 47, 22 & 2\\ 
       cmp    & 66 & 46, 20 & 2 \\ 
       diff   & 72 & 49, 23 & 2 \\ 
       patch   &69 & 47, 22 & 2\\
       bbox   & 69 & 47, 22& 2 \\
       toybox   & 67 & 46, 21 & 2\\
       sed & 69 & 47, 22 & 2\\ \bottomrule
    \end{tabular} 
        \end{footnotesize}
            \caption{MaxSAT solutions for the components in editors.}
    \label{tab:maxsateditors}
        \vspace{-0.5cm}
\end{table}



The algorithm first computes the scores of the seed configurations, inserts the 
pairs of seed configurations and their scores to a priority queue that orders 
according to non-decreasing score values. 
Then it executes $N$ fuzzing cycles, in each of which several mutations are performed 
according to the mode. 
We have been inspired by the fuzzing algorithm in AFL and included both deterministic and 
non-deterministic bit flips. We decided not to include bit insertions as we have a 
fixed input size, i.e., the number of configuration variables.
As a novelty, however, we have introduced interaction aware 
fuzzing, which chooses pairs of interacting configuration variables for simulatenous bit flipping. CONFIZZ can be easily extended to flip more than two interacting variables. 
After compleing the fuzzing cycles, the fuzzer returns $M$ of the generated configurations 
with the highest scores.


